Electroweak corrections to charged-current e+e- --> 4 fermion processes - technical details and further results

The complete electroweak O(alpha) corrections have been calculated for the charged-current four-fermion production processes e+e- --> nu_tau tau+ mu- anti-nu_mu, u anti-d mu- anti-nu_mu, and u anti-d s anti-c. Here, technical details of this calculation are presented. These include the algebraic reduction of spinor chains to a few standard structures and the consistent implementation of the finite width of the W boson. To this end, a generalization of the complex-mass scheme to the one-loop level is proposed, and the practical application of this method is described. Finally, the effects of the complete O(alpha) corrections to various differential cross sections of physical interest are discussed and compared to predictions based on the double-pole approximation, revealing that the latter approximation is not sufficient to fully exploit the potential of a future linear collider in an analysis of W-boson pairs at high energies.

==> Vertex-e-e-f1-f1-W.tex <==
{\small
\unitlength=1.2bp%

\begin{feynartspicture}(330,180)(4,2)

\FADiagram{}
\FAProp(0.,15.)(6.,15.)(0.,){/Straight}{-1}
\FALabel(3.,16.27)[b]{$e$}
\FAProp(0.,5.)(6.,5.)(0.,){/Straight}{1}
\FALabel(3.,3.93)[t]{$e$}
\FAProp(20.,15.)(14.,15.)(0.,){/Straight}{-1}
\FALabel(17.,16.07)[b]{$f_1$}
\FAProp(20.,10.)(14.,10.)(0.,){/Straight}{1}
\FALabel(17.,11.07)[b]{$f_2$}
\FAProp(20.,5.)(14.,5.)(0.,){/Sine}{-1}
\FALabel(17.,3.73)[t]{$W$}
\FAProp(6.,15.)(6.,5.)(0.,){/Straight}{-1}
\FALabel(4.93,10.)[r]{$\nu_e$}
\FAProp(6.,15.)(14.,15.)(0.,){/Sine}{-1}
\FALabel(10.,16.27)[b]{$W$}
\FAProp(6.,5.)(14.,5.)(0.,){/Sine}{1}
\FALabel(10.,3.93)[t]{$W$}
\FAProp(14.,15.)(14.,10.)(0.,){/Straight}{-1}
\FALabel(12.93,12.5)[r]{$f_2$}
\FAProp(14.,10.)(14.,5.)(0.,){/Sine}{0}
\FALabel(12.93,7.5)[r]{$\gamma/Z$}
\FAVert(6.,15.){0}
\FAVert(6.,5.){0}
\FAVert(14.,15.){0}
\FAVert(14.,10.){0}
\FAVert(14.,5.){0}

\FADiagram{}
\FAProp(0.,15.)(6.,15.)(0.,){/Straight}{-1}
\FALabel(3.,16.27)[b]{$e$}
\FAProp(0.,5.)(6.,5.)(0.,){/Straight}{1}
\FALabel(3.,3.93)[t]{$e$}
\FAProp(20.,15.)(14.,15.)(0.,){/Straight}{-1}
\FALabel(17.,16.07)[b]{$f_1$}
\FAProp(20.,10.)(14.,10.)(0.,){/Straight}{1}
\FALabel(17.,11.07)[b]{$f_2$}
\FAProp(20.,5.)(14.,5.)(0.,){/Sine}{-1}
\FALabel(17.,3.73)[t]{$W$}
\FAProp(6.,15.)(6.,5.)(0.,){/Straight}{-1}
\FALabel(4.93,10.)[r]{$e$}
\FAProp(6.,15.)(14.,15.)(0.,){/Sine}{0}
\FALabel(10.,16.27)[b]{$\gamma/Z$}
\FAProp(6.,5.)(14.,5.)(0.,){/Sine}{0}
\FALabel(10.,3.93)[t]{$\gamma/Z$}
\FAProp(14.,15.)(14.,10.)(0.,){/Straight}{-1}
\FALabel(12.93,12.5)[r]{$f_1$}
\FAProp(14.,10.)(14.,5.)(0.,){/Sine}{1}
\FALabel(12.93,7.5)[r]{$W$}
\FAVert(6.,15.){0}
\FAVert(6.,5.){0}
\FAVert(14.,15.){0}
\FAVert(14.,10.){0}
\FAVert(14.,5.){0}

\FADiagram{}
\FAProp(0.,15.)(6.,15.)(0.,){/Straight}{-1}
\FALabel(3.,16.27)[b]{$e$}
\FAProp(0.,5.)(6.,5.)(0.,){/Straight}{1}
\FALabel(3.,3.93)[t]{$e$}
\FAProp(20.,5.)(14.,5.)(0.,){/Straight}{-1}
\FALabel(17.,3.73)[t]{$f_1$}
\FAProp(20.,10.)(14.,10.)(0.,){/Straight}{1}
\FALabel(17.,11.07)[b]{$f_2$}
\FAProp(20.,15.)(14.,15.)(0.,){/Sine}{-1}
\FALabel(17.,16.07)[b]{$W$}
\FAProp(6.,15.)(6.,5.)(0.,){/Straight}{-1}
\FALabel(4.93,10.)[r]{$e$}
\FAProp(6.,15.)(14.,15.)(0.,){/Sine}{0}
\FALabel(10.,16.27)[b]{$\gamma/Z$}
\FAProp(6.,5.)(14.,5.)(0.,){/Sine}{0}
\FALabel(10.,3.93)[t]{$\gamma/Z$}
\FAProp(14.,5.)(14.,10.)(0.,){/Straight}{-1}
\FALabel(12.73,7.5)[r]{$f_1$}
\FAProp(14.,10.)(14.,15.)(0.,){/Sine}{1}
\FALabel(12.73,12.5)[r]{$W$}
\FAVert(6.,15.){0}
\FAVert(6.,5.){0}
\FAVert(14.,5.){0}
\FAVert(14.,10.){0}
\FAVert(14.,15.){0}

\FADiagram{}

\FADiagram{}
\FAProp(0.,15.)(5.,15.)(0.,){/Straight}{-1}
\FALabel(2.5,16.27)[b]{$e$}
\FAProp(0.,5.)(5.,5.)(0.,){/Straight}{1}
\FALabel(2.5,3.93)[t]{$e$}
\FAProp(20.,15.)(15.,15.)(0.,){/Straight}{-1}
\FALabel(17.5,16.07)[b]{$f_1$}
\FAProp(20.,5.)(15.,5.)(0.,){/Straight}{1}
\FALabel(17.5,3.73)[t]{$f_2$}
\FAProp(20.,10.)(5.,10.)(0.,){/Sine}{-1}
\FALabel(12.5,8.73)[t]{$W$}
\FAProp(5.,15.)(15.,15.)(0.,){/Sine}{-1}
\FALabel(10.,16.27)[b]{$W$}
\FAProp(5.,15.)(5.,10.)(0.,){/Straight}{-1}
\FALabel(3.73,12.5)[r]{$\nu_e$}
\FAProp(5.,5.)(15.,5.)(0.,){/Sine}{0}
\FALabel(10.,3.93)[t]{$\gamma/Z$}
\FAProp(5.,5.)(5.,10.)(0.,){/Straight}{1}
\FALabel(3.73,7.5)[r]{$e$}
\FAProp(15.,15.)(15.,5.)(0.,){/Straight}{-1}
\FALabel(14.23,12.5)[r]{$f_2$}
\FAVert(5.,15.){0}
\FAVert(5.,5.){0}
\FAVert(15.,15.){0}
\FAVert(15.,5.){0}
\FAVert(5.,10.){0}

\FADiagram{}
\FAProp(0.,15.)(6.,15.)(0.,){/Straight}{-1}
\FALabel(3.,16.27)[b]{$e$}
\FAProp(0.,5.)(6.,5.)(0.,){/Straight}{1}
\FALabel(3.,3.93)[t]{$e$}
\FAProp(20.,15.)(14.,15.)(0.,){/Straight}{-1}
\FALabel(17.,16.07)[b]{$f_1$}
\FAProp(20.,5.)(14.,5.)(0.,){/Straight}{1}
\FALabel(17.,3.73)[t]{$f_2$}
\FAProp(20.,10.)(14.,10.)(0.,){/Sine}{-1}
\FALabel(17.,11.07)[b]{$W$}
\FAProp(6.,15.)(6.,5.)(0.,){/Straight}{-1}
\FALabel(4.93,10.)[r]{$e$}
\FAProp(6.,15.)(14.,15.)(0.,){/Sine}{0}
\FALabel(10.,16.27)[b]{$\gamma/Z$}
\FAProp(6.,5.)(14.,5.)(0.,){/Sine}{0}
\FALabel(10.,3.93)[t]{$\gamma/Z$}
\FAProp(14.,15.)(14.,10.)(0.,){/Straight}{-1}
\FALabel(12.73,12.5)[r]{$f_1$}
\FAProp(14.,5.)(14.,10.)(0.,){/Straight}{1}
\FALabel(12.73,7.5)[r]{$f_2$}
\FAVert(6.,15.){0}
\FAVert(6.,5.){0}
\FAVert(14.,15.){0}
\FAVert(14.,5.){0}
\FAVert(14.,10.){0}

\FADiagram{}

\FADiagram{}
\end{feynartspicture}
}

